Multilingual Modal Sense Classification using a Convolutional Neural Network

Modal sense classification (MSC) is a special WSD task that depends on the meaning of the proposition in the modal's scope. We explore a CNN architecture for classifying modal sense in English and German. We show that CNNs are superior to manually designed feature-based classifiers and a standard NN classifier. We analyze the feature maps learned by the CNN and identify known and previously unattested linguistic features. We benchmark the CNN on a standard WSD task, where it compares favorably to models using sense-disambiguated target vectors.

==> results.tex <==
\section{Analysis and Discussion}
\paragraph{English}
\begin{itemize}
\item impact of word vectors for cnn and nn (what is the best per mv, are tuned or static better, how big are differences) (Table \ref{tbl:wordvectors} and \ref{tbl:wordvectorsbasic})

\item when did we beat majority baseline and CL2UBA? (micro avg) (Table \ref{tbl:resultsmpqa})

\item what happened with difficult genres for CL2UBA in MASC

\item top ngrams; comment statistics: location of ngrams in sentence and distance from mv; if we learned something meaningful extract it

\item what was misclassified

\item what happens when we ignore mv

\item we tried merging train data; very bad

\end{itemize}

\paragraph{German}

\begin{itemize}

\item impact of word vectors for cnn and nn

\item compare cnn and nn with default params

\item top ngrams investigation 

\item what was misclassified

\item what happens when we ignore mv

\item analyse difficult sense distinctions: are these the same as for E?

\item do the chosen features model comparable information to E? (can only investigate samples)

\item no identification of target, source and other dependents (restrictors)  $\Rightarrow$ future work, RNNs?; 

\item open: how well does CNN cope with a more difficult language such as German?

\item open: how well does CNN cope with difficult text genres?
\end{itemize}

==> tables/mpqa_results_save.tex <==
$\begin{table}[H]
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
            & can & could & may & must & should & micro\\
\midrule
BL$_{rand}$ & 33.33 & 33.33 & 50.00 & 50.00 & 50.00 & 41.49\\
MaxEnt & 59.64 & 61.25 & 92.14 & 87.60 & 90.11 & 74.88\\
NN & 56.01 & 55.42 & 90.00 & 75.24 & 88.68 & 69.74 \\ 
\midrule
CNN & \underline{\textbf{65.78}} & \underline{\textbf{67.50}} & \textbf{93.57} & \textbf{93.82} & \textbf{90.77} & \underline{\textbf{79.29}}\\
\bottomrule
\end{tabular}
\caption{Overall results comparison for classifiers trained on the \textbf{balanced} dataset. Modal verb is \textbf{not} ignored in a sentence. For a word representation, for every modal verb are chosen vectors which yielded the best results (Tables \ref{tbl:wordvectors} and \ref{tbl:wordvectorsbasic}). Scores of CNN which are significantly better (by conducting the mid-p-value McNemar test with p $\leq$ 0.05) than the next lower score are \underline{underlined}. }
\label{tbl:resultsba}
\end{table}

\begin{table}[H]
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
            & can & could & may & must & should & micro\\
\midrule
BL$_{major}$ & 69.92 & 65.00 & 93.57 & 94.32 & 90.81 & 80.18   \\
MaxEnt & 64.76 & 63.33 & 92.14 & 92.78 & \textbf{91.48} & 78.01\\
NN & 67.29 & 66.08 & \underline{\textbf{94.23}} & 86.37 & 90.96 & 77.93 \\ 
\midrule
CNN & $\overline{\textbf{70.87}}$ & \textbf{66.55} & 93.49 & \textbf{94.97} & 90.59 & \textbf{80.74}\\
\bottomrule
\end{tabular}
}
\caption{Overall results comparison for classifiers trained on the \textbf{unbalanced} dataset. Modal verb is \textbf{not} ignored in a sentence. For a word representation, for every modal verb are chosen vectors which yielded the best results (Tables \ref{tbl:cnnuba} and \ref{tbl:nnuba}). Scores of CNN which are significantly better (by conducting the mid-p-value McNemar test with p $\lrange$ 0.05) than the next lower score are \underline{underlined}. If CNN does not yield the best results, significance between the baseline having the best score and CNN is reported. $\overline{\text{Overlining}}$ is used if CNN with the unbalanced training performs significantly better than with the balanced training, and vice versa. } 
\label{tbl:resultsuba}
\end{table}


\begin{table}[H]
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{@{}ccccccc@{}}
\toprule
            & can & could & may & must & should & micro\\
\midrule
BL$_{major}$ & 33.33 & 33.33 & 50.00 & 50.00 & 50.00 & 81.33   \\
MaxEnt & 32.97 & 37.50 & 49.23 & 74.54 & 51.73 & 79.04 \\
NN & 34.41 & 41.73 & 42.75 & 56.8 & 51.73 & 76.53 \\ 
\midrule
CNN & 33.33 & 37.03 &50.00 & 67.36&50.00 & 81.74\\
\bottomrule
\end{tabular}
}
\caption{Overall results comparison for classifiers trained on the \textbf{unbalanced} dataset. Balanced accuracy is reported. } 
\label{tbl:balancedresults}
\end{table}

==> tables/wordvectorbasic.tex <==
\begin{table}[t]
\centering
\small
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{@{}c|c|c|c|c|c@{}}
%\begin{tabular}{c|c|c|c|c|c}
\toprule
\multicolumn{1}{r}{}& \multicolumn{1}{r}{can}& \multicolumn{1}{r}{could} & \multicolumn{1}{r}{may} & \multicolumn{1}{r}{must} & \multicolumn{1}{r}{should}\\
\midrule
    w2v-tuned & 63.18 & \textbf{57.07}  & 81.11 & 93.95 &  \textbf{90.59}\\ 
    dep-tuned & 62.43 & 53.74  & \textbf{83.20} & 93.95 & 90.23 \\
    rand-tuned & \textbf{67.29} & 56.16 & 79.42 & 93.95  & 89.87 \\
\bottomrule
\end{tabular}
}

\caption{Average accuracy of {\em NN}$_{EPOS_E + MPQA}$, 5-fold CV with different input representation.}
\label{tbl:wordvectorsbasic}
\end{table}

